Learning to Remember: A Synaptic Plasticity Driven Framework for Continual Learning

Models trained in the context of continual learning (CL) should be able to learn from a stream of data over an undefined period of time. The main challenges herein are: 1) maintaining old knowledge while simultaneously benefiting from it when learning new tasks, and 2) guaranteeing model scalability with a growing amount of data to learn from. In order to tackle these challenges, we introduce Dynamic Generative Memory (DGM) - a synaptic plasticity driven framework for continual learning. DGM relies on conditional generative adversarial networks with learnable connection plasticity realized with neural masking. Specifically, we evaluate two variants of neural masking: applied to (i) layer activations and (ii) to connection weights directly. Furthermore, we propose a dynamic network expansion mechanism that ensures sufficient model capacity to accommodate for continually incoming tasks. The amount of added capacity is determined dynamically from the learned binary mask. We evaluate DGM in the continual class-incremental setup on visual classification tasks.

==> sections/preliminaries.tex <==



Adopting the notation of \cite{RWalk}, let  $S_{t}=\{(x_{i}^{t}, \textit{y}_{i}^{t} )\}_{i=1}^{n^{t}} $ denote a collection of data belonging to the task $t \in T$, where $x_i^t \in \mathcal{X}$ is the input data and $\textit{y}_i^t \in \boldmath{\textit{y}^t}$ are the ground truth labels. While in the (standard) non-incremental setup the entire dataset $S =\cup_{t=0}^{|T|}S_{t}$ is available at once, in an incremental setup %
it becomes available to the model in chunks $S_t$ specifically only during the learning of task $t$.  Thereby, $S_{t}$ can be composed of a collection of items from different classes, or even from a single class only. %
Furthermore, during test time the output space covers all the labels observed so far featuring the single head evaluation: %
$ \mathcal{Y}^t = \cup_{j=1}^{t}\textit{y}^j$.  %



 















